How good is good enough for COVID19 apps? The influence of benefits, accuracy, and privacy on willingness to adopt

A growing number of contact tracing apps are being developed to complement manual contact tracing. A key question is whether users will be willing to adopt these contact tracing apps. In this work, we survey over 4,500 Americans to evaluate (1) the effect of both accuracy and privacy concerns on reported willingness to install COVID19 contact tracing apps and (2) how different groups of users weight accuracy vs. privacy. Drawing on our findings from these first two research questions, we (3) quantitatively model how the amount of public health benefit (reduction in infection rate), amount of individual benefit (true-positive detection of exposures to COVID), and degree of privacy risk in a hypothetical contact tracing app may influence American's willingness to install. Our work takes a descriptive ethics approach toward offering implications for the development of policy and app designs related to COVID19.

==> citations.tex <==
3The Impact of Perceived Privacy, Accuracy and Security on the Adoption of Mobile Self-Checkout Systems


% Privacy Only

The impact of privacy concern on user adoption of location‐based services


% Accuracy Only

Accuracy and Adoption of Wearable Technology Used by Active Citizens: A Marathon Event Field Study

% Adoption of serives with Accuracy and Privacy concerns
The Adoption and Implementation of RFID Technologies in Healthcare: A Literature Review
    https://link.springer.com/article/10.1007/s10916-011-9789-8

Wearable activity trackers, accuracy, adoption, acceptance and health impact: A systematic literature review

Adoption Criteria Evaluation of Activity Tracking
Wristbands for University Students

A user study on the adoption of location based services
